The graph alignment problem: fundamental limits and efficient algorithms

This thesis studies the graph alignment problem, the noisy version of the graph isomorphism problem, which aims to find a matching between the nodes of two graphs which preserves most of the edges. Focusing on the planted version where the graphs are random, we are interested in understanding the fundamental information-theoretical limits for this problem, as well as designing and analyzing algorithms that are able to recover the underlying alignment in the data. For these algorithms, we give some high probability guarantees on the regime in which they succeed or fail.

==> overview_fr.tex <==
\subsubsection{Présentation générale}
Cette thèse a pour contexte l'inférence statistique sur des graphes (ou matrices) en grande dimension et étudie le problème d'alignement de graphes, qui consiste à retrouver un appariement sous-jacent entre les sommets de deux graphes aléatoires correlés.

Comme pour de nombreux problèmes d'inférence dans des modèles dit plantés, nous nous intéressons aux limites fondamentales ainsi qu'à la difficulté computationnelle du problème.

Nous étudions tout d'abord un modèle gaussien dans lequel les graphes sont complets et où les poids des arêtes matchées sous la  correspondence sous-jacente sont corrélées. Nous établissons un seuil informationnel pour la tâche d'alignement exact dans ce modèle, et étudions un algorithme spectral simple, \alg{EIG1}, consistant à aligner les vecteurs propres dominants des matrices d'adjacence des deux graphes.

Tandis que la grande majorité des travaux récents sur le sujet est dédiée à l'alignement exact dans les graphes denses, nous explorons dans la suite de la thèse un régime dit parcimonieux dans lequel le degré moyen des sommets est constant, indépendant de la taille du graphe. Pour les graphes  d'Erd\H{o}s-R\'enyi, dans ce régime ou l'alignment est plus difficile, n'importe quel algorithme ne pourra aligner seulement qu'une fraction des noeuds : on parle d'alignement partiel. Nous démontrons un résultat informationnel caractérisant un régime dans lequel l'alignement partiel est impossible, et donnant une borne supérieure sur la fraction de noeuds du graphe qu'un estimateur peut espérer correctement aligner.

Nous proposons par la suite un algorithme, \alg{NTMA}, pour l'alignement partiel dans le régime où les graphes sont parcimonieux, définissant une mesure de similarité -- appelée \emph{tree matching weight} -- entre les voisinages arborescents des sommets des deux graphes.

En étudiant l'alignement de graphes parcimonieux d'un point de vue local, un autre problème associé apparaît : la détection de corrélation dans les arbres. Ce problème de test d'hypothèses, non étudié auparavant, consiste à décider si deux arbres aléatoires sont corrélés ou indépendants. Le \emph{tree matching weight} donne une première méthode pour résoudre ce problème; dans une autre contribution, nous étudions un test optimal pour cette tâche de détection, basé sur le rapport de vraisemblance. Dans un modèle d'arbres de Galton-Watson corrélés, qui sont bien connus pour être les approximations locales des graphes d'Erd\H{o}s-R\'enyi parcimonieux, nous caractérisons le régime de performance de ce test. 

L'étude de ce problème sur les arbres donne ainsi naturellement un algorithme de passage de messages en temps polynomial pour notre tâche initiale d'alignement de graphes: \alg{MPAlign}. Nous prouvons que cette méthode retrouve une fraction du signal planté dans certains régimes de paramètres. A la fin de la thèse, nous incluons des résultats récents qui affinent considérablement l'analyse du problème de détection de corrélation dans les arbres : nous exhibons une transition de phase asymptotique en le paramètre de corrélation $s$ qui gouverne la faisabilité ou l'impossibilité de cette tâche de détection, et partant précise les régimes dans lesquels \alg{MPAlign} est performant. Le régime où l'approche locale ne permet pas de retrouver une fraction du signal planté semble indiquer la présence d'une phase difficile pour l'alignement de graphes parcimonieux, ce que nous conjecturons.

\subsubsection{Chapitre 1 -- Introduction} Ce chapitre introductif est une présentation générale des motivations, objets, outils, et questions discutés dans cette thèse. 
Devant l'importance croissante de la représentation des données sous forme de graphes dans une variété de domaines, nous introduisons et motivons le cadre général de l'inférence statistique sur des graphes (ou matrices) en grande dimension. 

Dans son sens le plus large, l'inférence statistique vise à retrouver de l'information basées sur l'observation des données. Supposons que nous ayons à disposition des échantillons (vecteurs $\dR^d$, graphes, matrices, etc.) tirés selon une certaine distribution de probabilité. Le statisticien conçoit des méthodes pour récupérer des informations sur cette distribution de probabilité, par exemple en testant des hypothèses ou en dérivant des estimations pour un paramètre $\theta \in \Theta$ de la distribution. Le cadre habituel est le suivant :
$$\mbox{paramètre } \theta \in \Theta \longrightarrow \mbox{données }  Y  \longrightarrow \mbox{estimateur } \theta^*$$
Les principales questions (informelles) qui se posent dans ce cadre sont : "comment pouvons-nous discriminer différents modèles ou différentes hypothèses ?", ainsi que "pouvons-nous estimer efficacement le paramètre $\theta$ ?"

Un cadre commun à de nombreux problèmes d'inférence est celui dit des \emph{problèmes plantés}. Dans ce contexte, l'observation est pensée comme résultant de la perturbation aléatoire d'un signal sous-jacent d'intérêt. Décrivons formellement le modèle : un certain signal $X$ est tiré selon une certaine distribution a priori (nous travaillons donc dans un cadre bayésien), et est "planté" dans les données. Étant donné le signal $X$, l'observation $Y$ est tirée selon une certaine distribution conditionnelle $p(\cdot \, | \, X)$. Le cadre est le suivant :
$$\mbox{signal } X \sim p_X \longrightarrow \mbox{observation }  Y \sim p(\cdot \, | \, X)  \longrightarrow \mbox{estimateur } X^*$$

Les deux questions informelles mentionnées précédemment -- tester des hypothèses et estimer certains paramètres -- peuvent être reformulées dans ce contexte planté :
\begin{itemize}
\item[$(i)$] Pouvons-nous détecter la présence d'un signal planté dans les données ?
\item[$(ii)$] Si oui, sommes-nous également capables de reconstruire ce signal ?
\end{itemize}
Définissons $n$ comme le paramètre de dimension du problème (taille du graphe, de la matrice, nombre d'échantillons, etc.), de sorte que travailler dans le régime de grande dimension correspond à faire tendre $n$ vers l'infini.

La question $(i)$ ci dessous définit la tâche de \emph{détection}. Détecter la présence du signal consiste exactement à discriminer un modèle sans signal planté -- le modèle nul -- du modèle planté, sur la base de l'observation de $Y$, c'est-à-dire à résoudre le test d'hypothèse suivant :
$$ \cH_0 := \mbox{ "$Y$ est tiré selon le modèle nul"} \quad \mbox{contre} \quad \cH_1 := \mbox{ "$Y$ est tiré selon le modèle planté"}.$$
Pour une tâche de détection donnée, il s'agit concevoir un test $T$ (c'est-à-dire, une fonction mesurable de $Y$ prenant des valeurs dans $\set{0,1}$) pour lequel nous sommes capables de fournir des garanties avec une probabilité tendant vers $1$ asymptotiquement en $n$.

La question $(ii)$ définit la tâche de \emph{reconstruction}. Reconstruire le signal correspond à trouver un estimateur $\hat{X}$ (c'est-à-dire, une fonction mesurable de $Y$) pour lequel nous sommes capables de fournir des garanties (par exemple, prouver que $\hat{X}$ est proche de $X$ en un certain sens) avec une probabilité tendant vers $1$ asymptotiquement en $n$.

Le but de cette thèse est de comprendre les aspects fondamentaux de ces questions et de concevoir des algorithmes pour les tâches qu'elles requièrent. 
Dans la suite de l'introduction, nous passons en revue les concepts de base de la théorie des graphes aléatoires, et énonçons des résultats généraux qui seront utiles tout au long du manuscrit (voir partie 1.2.1). 

Nous donnons ensuite plusieurs exemples emblématiques de problèmes d'inférence dans les graphes aléatoires : la clique plantée, la détection de communautés, et le matching planté. Nous définissons les trois régimes (impossible, difficile, facile) correspondant aux tâches de détection ou de reconstruction, et illustrons la présence de transition de phase en grande dimension sur un exemple élémentaire (1.2.2, 1.2.3).

Enfin, nous donnons le cadre général de l'alignement de graphes, sujet central de cette thèse. Nous détaillons quelques unes des nombreuses applications de ce problème : la désanonymisation de données, le traitement d'image et reconnaissance de forme, la biologie computationnelle -- avec notamment l'inférence au sein des réseaux d'interaction protéïques -- ainsi que le traitement automatique du langage. Nous parcourons ensuite les résultats élémentaires généraux ainsi qu'une revue de littérature sur les techniques, méthodes et travaux théoriques antérieurs sur le sujet (1.3). Nous introduisons également le problème de détection de corrélation dans les arbres, qui sera abordé dans les chapitres 5, 6 et 7, ainsi qu'un résultat heuristique qui montre le lien profond entre les deux problèmes (1.4).

\subsubsection{Chapitre 2 -- Alignement de matrices gaussiennes : limites fondamentales} 
Ce chapitre, basé sur l'article \emph{Sharp threshold for alignment of graph databases with gaussian weights} \cite{Ganassali21MSML}, publié à \emph{MSML 2021}, étudie les limites fondamentales (informationnelles) pour l'alignement exact de graphes (ou matrices) $A,B$ dans le cadre où les arêtes sont pondérées par des gaussiennes corrélées. 

Nous considérons le modèle de Wigner de paramètres $n,\rho$ défini dans l'introduction (1.3), et nous prouvons qu'il existe un seuil dit \emph{sharp} pour la reconstruction exacte de $\pi^\star$. Le résultat est le suivant : si $n \rho^2 \geq (4+\eps) \log n + \omega(1)$  pour un certain $\eps>0$, il existe un estimateur $\hat{\pi}$ -- en l'espère, l'estimateur du maximum a posteriori -- basé sur l'observation des bases des matrices $A,B$ qui réalise une reconstruction exacte avec forte probabilité. En revanche, si $n \rho^2 \leq 4 \log n - \log \log n - \omega(1)$ alors tout estimateur $\hat{\pi}$ vérifie $\hat{\pi}= \pi^\star$ avec probabilité $o(1)$.

Ce résultat montre que le seuil informationnel pour l'alignement exact est le même que celui obtenu pour la détection dans \cite{Wu20} : en d'autres termes, pour l'alignement de graphes pondérés gaussiens, le problème de la reconstruction n'est fondamentalement pas plus difficile que celui de la détection.
Les preuves reposent sur l'analyse de l'estimateur du maximum a posteriori et de la méthode du second moment -- introduits précédemment dans la section 1.2.1 de l'introduction -- ainsi que sur l'étude de la structure de corrélation des énergies associées aux permutations.

\subsubsection{Chapitre 3 -- Alignement de matrices gaussiennes : analyse d'une méthode spectrale} Nous poursuivons l'exploration du cadre gaussien dans ce chapitre, en étudiant une méthode spectrale simple et naturelle pour la reconstruction, notée \alg{EIG1}. \'Etant donné les deux matrices d'adjacence $A$ et $B$ des deux graphes, \alg{EIG1} aligne leurs deux vecteurs propres principaux $v_1$ et $v'_1$, au signe près de $v'_1$.

Nous considérons le modèle gaussien de paramètres $n,\xi$ défini précédemment : $A$ appartient au $\GOE$ et est de taille $n \times n$, et $B$ est une version bruitée de $A$ où tous les noeuds ont été relabelisés selon une permutation plantée $\pi^\star$. Nous montrons la loi du zéro-un suivante : avec forte probabilité, sous la condition $\xi n^{7/6+\epsilon} \to 0$ pour un certain $\eps>0$, \alg{EIG1} reconstruit $\pi^\star$ à partie négligeable près, tandis que si $\xi n^{7/6-\epsilon} \to \infty$, cette méthode ne peut retrouver que $o(n)$ correspondances correctes.

Ce résultat donne une compréhension de la méthode spectrale la plus simple et la plus rapide pour l'alignement de matrices (ou l'alignement de graphes pondérés complets), et utilise des méthodes de preuve et des techniques d'intérêt plus large que le seul cadre de ce chapitre. Ce chapitre est basé sur l'article \textit{Spectral alignment of correlated gaussian matrices} \cite{GLM19}, publié dans \emph{Advances in Probability}.

\subsubsection{Chapitre 4 -- Alignement de graphes d'\ER parcimonieux : résultats informationnels} Nous nous focalisons dans ce chapitre sur l'étude de l'alignement de graphes d'\ER dans le régime parcimonieux, où le degré moyen des graphes $\lambda >0$ et la corrélation $s \in [0,1]$ sont des constantes (ne dépendant pas du nombre de noeuds). Basé sur l'article \emph{Impossibility of partial recovery in the graph alignment problem} \cite{ganassali2021impossibility} publié à \emph{COLT 2021}, nous prouvons un résultat informationnel caractérisant un régime où même un alignement partiel est impossible. 

Ce résultat prend la forme suivante : pour tout $\lambda>0$ et $s\in[0,1]$, on a, pour tout estimateur $\hat{\pi}$,
$$ \dP\left(\ov(\hat{\pi},\pi^{\star}) > (c(\lambda s)+ \eps) n  \right) \underset{n \to \infty}{\longrightarrow} 0 \quad \mbox{pour tout } \eps>0 \, , $$
où $c(\mu)$ est la fraction typique de sommets dans la composante géante d'un graphe d'\ER de degré moyen $\mu$. 
En particulier, comme $c(\mu)=0$ si $\mu \leq 1$, ce résultat implique l'impossibilité de la reconstruction partielle lorsque $\lambda s \leq 1$. De plus, si $\lambda s > 1$, nous avons établi que l'overlap réalisable par tout estimateur est borné supérieurement par $c(\lambda s) n+o(n)$.

La preuve de ce résultat repose sur une méthode probabiliste qui permute les petites composantes arborescentes du graphe intersection, et crée ainsi artificiellement de nombreux autres candidats pour $\pi^\star$, de probabilité à posteriori égales à celles de $\pi^\star$, et donc indistinguables pour le statisticien. 

\subsubsection{Chapitre 5 -- Mesurer la similarité entre arbres pour l'alignement de graphes parcimonieux} Nous poursuivons dans ce chapitre l'étude de l'alignement de graphes parcimonieux, cette fois-ci du point de vue algorithmique.

Nous introduisons le \emph{Neighborhood Tree Matching Algorithm} (\alg{NTMA}), basé sur une mesure de similarité entre les arbres. Pour les graphes aléatoires d'\ER corrélés, nous prouvons que l'algorithme retourne -- en temps polynomial -- une fraction positive de sommets correctement appariés, et une fraction négligeable de mauvaises paires. Ce résultat est valable avec un degré moyen des graphes en $O(1)$ et un paramètre de corrélation $s$ qui peut être constant et borné loin de $1$, des conditions dans lesquelles l'alignement de graphes aléatoires est particulièrement difficile. 

\alg{NTMA} repose sur une mesure de similarité -- appelée \emph{poids d'alignement d'arbres} -- entre les voisinages arborescents des nœuds dans les graphes. Pour deux arbres non étiquetés $t$ et $t'$ de profondeur supérieure ou égale à $d$, le poids d'alignement $\cW_d(t,t')$ entre $t$ et $t'$ à profondeur $d$ est le nombre maximal de sommets à profondeur exactement $d$ d'un sous-arbre (non étiqueté) commun à $t$ et à $t'$. D'un point de vue computationnel, ces poids vérifient des relations de récurrence de type max-somme qui permettent de les calculer efficacement lorsque $d$ ne croît pas trop vite, via des méthodes dynamiques. 

En étudiant le comportement de cette métrique de correspondance pour plusieurs modèles d'arbres aléatoires corrélés, nous parvenons à donner des garanties pour que cette quantité discrimine efficacement les voisinages de paires de sommets $(u,u')$ en correspondance ($u' = \pi^\star(u)$) de paires de sommets distincts ($u' \neq \pi^\star(u)$).

Ces résultats présentent un intérêt plus général, au delà du cadre de l'alignement de graphes. En particulier ils donnent une méthode de test efficace pour déterminer si deux arbres aléatoires sont corrélés ou indépendants.
 
Ce chapitre est basé sur l'article \emph{From tree matching to sparse graph alignment} \cite{Ganassali20a}, publié à \emph{COLT 2020}.

\subsubsection{Chapitre 6 -- Détection de corrélation dans des arbres} Nous suivons l'approche locale précédente dans le régime parcimonieux et nous intéressons plus en détail à la détection de corrélation dans les arbres aléatoires non étiquetés. 

Plus précisément nous considérons le problème de test d'hypothèses où sous $\cH_0$ les arbres sont des arbres indépendants de Galton-Watson et dont la loi de reproduction est $\Poi(\lambda)$, et sous $\cH_1$ les deux arbres ont mêmes lois marginales que sous $\cH_0$, mais contiennent un sous arbre commun lui aussi Galton-Waston de loi de reproduction $\Poi(\lambda s)$, et sont ainsi corrélés. Ce modèle de Galton-Watson corrélé est bien connu pour être l'approximation locale du modèle d'\ER corrélé parcimonieux.

A profondeur fixée $d$, la théorie de Neyman-Pearson fournit naturellement un estimateur optimal pour notre tâche basé sur le rapport de vraisemblance, $\cL_d(t,t')$. Là encore, $\cL_d(t,t')$ satisfait une relation de récurrence qui permet son calcul par des méthodes dynamiques lorsque $d$ ne croît pas trop vite. 
Nous caractérisons certains régimes de paramètres $(\lambda,s)$ où ce test fonctionne, et à l'inverse certains autres où il échoue. 

Ensuite, nous montrons une connexion forte entre le problème de détection de corrélation dans des arbres et celui de l'alignement de graphes. Dans ce dernier, nous proposons un algorithme de \emph{message-passing}, \alg{MPAlign}, consistant à calculer, pour chaque paire de sommets $u$ dans $\cG$ et $u'$ dans $\cH$, la quantité $\cL_d(t_u,t'_{u'})$ où $t_u$ (respectivement $t'_{u'}$) est le voisinage arborescent à profondeur $d$ du sommet $u$ dans $\cG$ (respectivement de $u'$ dans $\cH$). Nous prouvons ainsi que dès lors que le test basé sur $\cL_d(t,t')$ parvient à discriminer $\cH_1$ de $\cH_0$, alors l'algorithme \alg{MPAlign} reconstruit partiellement la permutation plantée $\pi^\star$.   Cet algorithme de transmission de messages est analysé et récupère de manière prouvée une fraction du signal planté dans certains régimes de paramètres. Le chapitre est basé sur l'article \emph{Correlation detection in trees for partial graph alignment} \cite{GMLTrees2021journal}, soumis à \emph{Annals of Applied Probability}. Une version courte de ce travail, sous un nom légèrement différent, \emph{Correlation Detection in Trees for Planted Graph Alignment} \cite{GMLTrees2021ITCS} est parue à \emph{ITCS 2021}.

\subsubsection{Chapitre 7 -- Addendum : nouveaux résultats pour la détection de corrélation dans des arbres} Nous avons ajouté un dernier chapitre à la fin de la thèse, présentant des résultats récents pour la détection de corrélation dans les arbres. Ces résultats améliorent considérablement les travaux antérieurs et fournissent une compréhension générale des limites fondamentales du problème, ainsi que quelques perspectives intéressantes discutées par la suite dans la conclusion. Nous prouvons que le problème de détection de corrélation dans les arbres, dans un régime où la profondeur tend vers l'infini, présente une transition abrupte en le paramètre $s$, asymptotiquement en $\lambda$, comme énoncé ci-dessous.

Si l'on note $A_n$ le nombre d'arbres enracinés et non étiquetés à $n$ sommets. Otter a démontré en 1948 \cite{Otter48} un equivalent de cette quantité lorsque $n$ est grand :
$$A_n \underset{n \to \infty}{\sim} \frac{D}{n^{3/2}} \left( \frac{1}{\alpha} \right)^n, $$
pour un certain $D>0$, où $\alpha \in (0,1)$ est appelée \emph{constante d'Otter}, et vaut numériquement $\alpha \sim 0.3383$. Cette constante joue un rôle fondamental dans notre problème, comme décrit ci-après :
\begin{itemize}
\item[$(i)$] (résultat négatif) Si $s \leq \sqrt{\alpha} \sim 0.5816$, alors pour tout $\lambda>0$, la détection de corrélation dans les grands arbres de Galton-Watson corrélés est impossible.
\item[$(ii)$] (résultat positif) Si $s > \sqrt{\alpha} \sim 0.5816$, alors il existe $\lambda(s)>0$ tel que pour tout $\lambda \geq \lambda(s)$, le test basé sur $\cL_d(t,t')$ est efficace : la détection de corrélation dans les grands arbres de Galton-Watson corrélés est possible.
\end{itemize}

Ce résultat montre donc la présence d'une transition de phase asymptotique en le paramètre de corrélation $s$ qui gouverne la faisabilité ou l'impossibilité de cette tâche de détection, et partant précise les régimes dans lesquels \alg{MPAlign} est performant. Le régime où l'approche locale ne permet pas de retrouver une fraction du signal planté semble indiquer la présence d'une phase difficile pour l'alignement de graphes parcimonieux, ce que nous conjecturons.

\subsubsection{Aperçu des questions ouvertes}
Le manuscrit se conclut par une conclusion qui, après avoir rappelé les approches et résultats, mentionne quelques questions ouvertes et directions de recherche qui nous semblent particulièrement intéressantes. Nous en donnons ci-après un aperçu non exhaustif.

\subsubsection*{Valeurs typiques du QAP dans le modèle nul}
Nous rappelons que la version non plantée de l'alignement de deux graphes avec matrices d'adjacence $A$ et $B$ consiste à résoudre le problème d'assignation quadratique $\max_\Pi \langle A, \Pi B \Pi^T\rangle$. Une question d'intérêt est alors de comprendre la valeur de et objectif dans la limite de grande taille dans le modèle nul, par exemple lorsque $A,B$ sont des graphes d'\ER indépendants. Certaines bornes supérieures existent dans la littérature \cite{Wu20} -- pour étudier le problème de détection -- mais à notre connaissance, la valeur exacte de cet objectif n'est pas connue.

\subsubsection*{Fraction optimale pour la reconstruction partielle}
Un problème encore ouvert est celui de déterminer la plus grande fraction des sommets -- ou, le plus grand sous-ensemble $\cC$ -- que l'on peut espérer aligner dans le régime parcimonieux. Il est démontré dans le Chapitre \ref{chapter:impossibility} que -- à fraction négligeable des nœuds près -- cet ensemble $\cC$ est contenu dans le composant géant $\cC_1$ du graphe intersection sous-jacent. Dans la Section \ref{subsection:warmup}, nous avons traité le cas d'isomorphisme exact $s=1$, pour lequel $\cC$ est à fraction négligeable près l'ensemble de tous les points invariants par l'action du groupe des automorphismes. Nous conjecturons que cette observation pourrait être généralisée au cas non-isomorphe $s <1$, à savoir que $\cC$ est là encore à fraction négligeable près l'ensemble $\cI$ des nœuds invariants par l'action du groupe des automorphismes \emph{dans le graphe intersection}.

\subsubsection*{Difficulté computationnelle}
D'autres branches actives de la recherche donnent des éclairages sur la difficulté computationnelle des problèmes d'inférence (voir \cite{Bubeck18} pour une approche basée sur la réduction). Obtenir des résultats plus quantitatifs sur la difficulté de l'alignement de graphes est encore une question ouverte : plusieurs pistes pourraient d'être explorées. La méthode des faibles degré (\emph{low-degree}) \cite{Kunisky19} suggère que la projection du rapport de vraisemblance dans l'espace des polynômes de faible degré donne de solides indications sur la faisabilité en temps polynomial d'un problème de détection. Mentionnons également une autre méthode issue de la théorie des verres de spin, la propriété d'\emph{overlap gap property}, qui est établie pour révéler la difficulté algorithmique dans les problème d'optimisation combinatoire et l'inférence dans les modèles plantés -- celle, en fait, des algorithmes locaux. Elle a récemment été démontrée pour le problème de la clique plantée \cite{Gamarnik2019TheLO} et pourrait être étudie dans le cas de l'alignement de graphes.

